Controlled Neural Sentence-Level Reframing of News Articles

Framing a news article means to portray the reported event from a specific perspective, e.g., from an economic or a health perspective. Reframing means to change this perspective. Depending on the audience or the submessage, reframing can become necessary to achieve the desired effect on the readers. Reframing is related to adapting style and sentiment, which can be tackled with neural text generation techniques. However, it is more challenging since changing a frame requires rewriting entire sentences rather than single phrases. In this paper, we study how to computationally reframe sentences in news articles while maintaining their coherence to the context. We treat reframing as a sentence-level fill-in-the-blank task for which we train neural models on an existing media frame corpus. To guide the training, we propose three strategies: framed-language pretraining, named-entity preservation, and adversarial learning. We evaluate respective models automatically and manually for topic consistency, coherence, and successful reframing. Our results indicate that generating properly-framed text works well but with tradeoffs.

==> table-reframing-example-full-c.tex <==
\begin{table}[t!]

\small
\centering
%\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{2pt}

\begin{tabular}{p{0.98\linewidth}}
\toprule
{Original text} \\
\midrule
All that was true of interracial marriages shortly after World War II. 
\textbf{Today, interracial marriage has strong public support, and no successful politician or prominent public figure favors outlawing such unions.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (q)~GPT-2 + $\strategy_{\rm F}$} (crime-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{Actually, a number of people within a decade may have wanted to apply for visas. The ''Hispanic} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (r)~$\strategy_{\emptyset}$} (crime-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{Bob Greene: gay marriage is on the same trajectory or so fundamentally different that it will never be legalized. He says if it's legalized, it'll be a reversal of the trend.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (s)~B.Coherence} (crime-reframed text) \\
\midrule
All that was true of interracial marriages shortly after World War II. 
\textbf{Today, interracial marriages have become a rite of passage for gays and lesbians alike, but they're not legal.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (t)~B.Framing} (crime-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{''It's not a crime,'' he said, but it's a felony, and he's innocent.''} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (u)~B.Balance} (crime-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{Today, the nation's highest court ruled that anyone who commits a crime with a gun should be spared the death penalty.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\bottomrule
\end{tabular}

\caption{
(a)~Sample text from the media frames corpus. The bold sentence is labeled with the {\em policy} frame.
(q-u)~Reframed sentences with the five manual labeled approaches to the {\em crime} frame.}
\label{table-reframing-example-full}

\end{table}


	



==> table-reframing-example-full-e.tex <==
\begin{table}[t!]

\small
\centering
%\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{2pt}

\begin{tabular}{p{0.98\linewidth}}
\toprule
{Original text} \\
\midrule
All that was true of interracial marriages shortly after World War II. 
\textbf{Today, interracial marriage has strong public support, and no successful politician or prominent public figure favors outlawing such unions.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (b)~GPT-2 + $\strategy_{\rm F}$} (economic-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{Actually, a number of people within a decade may have wanted to apply for visas. The ''Hispanic} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (c)~$\strategy_{\emptyset}$} (economic-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{Bob Greene: Gay marriage is on the same trajectory as interracial marriage. He says it is so fundamentally different that it will never be legalized.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (d)~B.Coherence} (economic-reframed text) \\
\midrule
All that was true of interracial marriages shortly after World War II. 
\textbf{Today, same-sex marriages are legal in many states, but they are not as legal as interracial marriages, according to a new study.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (e)~B.Framing} (economic-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{''It's a good thing that we're able to do this,'' said a spokesman for the tobacco industry, who is suing the tobacco companies.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (f)~B.Balance} (economic-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{Today's tight labor market dictates that employers consider workers based on the skills they possess rather than the partners they prefer. Gay couples must also consider the financial obligations they owe their employers, he says.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
\bottomrule
\end{tabular}

\caption{
(a)~Sample text from the media frames corpus. The bold sentence is labeled with the {\em policy} frame.
(b-e)~Reframed sentences with the five manual labeled approaches to the {\em economic} frame.}
\label{table-reframing-example-full-e}

\end{table}


	



==> table-reframing-example-full-l.tex <==
\begin{table}[t!]

\small
\centering
%\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{2pt}

\begin{tabular}{p{0.98\linewidth}}
\toprule
{Original text} \\
\midrule
All that was true of interracial marriages shortly after World War II. 
\textbf{Today, interracial marriage has strong public support, and no successful politician or prominent public figure favors outlawing such unions.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (g)~GPT-2 + $\strategy_{\rm F}$} (legality-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{It was St. Louis' law in February 1992 that stood the test of time for the Court when} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (h)~$\strategy_{\emptyset}$} (legality-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{Interracial marriages were legalized in the United States after the Second World War, but today it's a question of whether it will ever be legalized.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (i)~B.Coherence} (legality-reframed text) \\
\midrule
All that was true of interracial marriages shortly after World War II. 
\textbf{Today, same-sex marriages are legalized, but only a fraction of them have been legalized in this country.''} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (j)~B.Framing} (legality-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{''It's a very sad day,'' he said, referring to the state's ban on same-sex marriage.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (k)~B.Balance} (legality-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{Today, it's a battle for a constitutional amendment that would ban gay marriage but allow same-sex couples to enter into civil unions.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\bottomrule
\end{tabular}

\caption{
(a)~Sample text from the media frames corpus. The bold sentence is labeled with the {\em policy} frame.
(g-k)~Reframed sentences with the five manual labeled approaches to the {\em legality} frame.}
\label{table-reframing-example-full-l}

\end{table}


	



==> table-reframing-example-full-p.tex <==
\begin{table}[t!]

\small
\centering
%\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{2pt}

\begin{tabular}{p{0.98\linewidth}}
\toprule
{Original text} \\
\midrule
All that was true of interracial marriages shortly after World War II. 
\textbf{Today, interracial marriage has strong public support, and no successful politician or prominent public figure favors outlawing such unions.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (l)~GPT-2 + $\strategy_{\rm F}$} (policy-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{Or if they feel it is not in their interests to simply veto legislation sponsored by the other party and} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (m)~$\strategy_{\emptyset}$} (policy-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized, says aaron carroll.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (n)~B.Coherence} (policy-reframed text) \\
\midrule
All that was true of interracial marriages shortly after World War II. 
\textbf{Today, same-sex marriage is legal, but it's a far cry from what's been said of the civil rights movement.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (o)~B.Framing} (policy-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{''It's a good idea,'' said Sen. John McCain, D-N.Y., a Democrat who voted for the measure.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\addlinespace
\midrule
{\bfseries (p)~B.Balance} (policy-reframed text) \\
All that was true of interracial marriages shortly after World War II. 
\textbf{Today's debate over whether the death penalty is imposed fairly and impartially enough to suit not the legal but the moral conscience of the nation's citizens is raging.} 
The question is whether gay marriage is on the same trajectory or is so fundamentally different that it will never be legalized.\\
\bottomrule
\end{tabular}

\caption{
(a)~Sample text from the media frames corpus. The bold sentence is labeled with the {\em policy} frame.
(l-p)~Reframed sentences with the five manual labeled approaches to the {\em policy} frame.}
\label{table-reframing-example-full-p}

\end{table}


	


